TextureGAN: Controlling Deep Image Synthesis with Texture Patches

In this paper, we investigate deep image synthesis guided by sketch, color, and texture. Previous image synthesis methods can be controlled by sketch and color strokes but we are the first to examine texture control. We allow a user to place a texture patch on a sketch at arbitrary locations and scales to control the desired output texture. Our generative network learns to synthesize objects consistent with these texture suggestions. To achieve this, we develop a local texture loss in addition to adversarial and content loss to train the generative network. We conduct experiments using sketches generated from real images and textures sampled from a separate texture database and results show that our proposed algorithm is able to generate plausible images that are faithful to user controls. Ablation studies show that our proposed pipeline can generate more realistic images than adapting existing methods directly.

==> application.tex <==
\section{Application}

Talk about the app Varun is working on. Show some screenshot here?

==> figures/fig-DTD-with-segmentation.tex <==
\begin{figure}[htb]
  \centering
  \includegraphics[width=\linewidth]{images/local_vs_global.pdf}
  \caption{\patsorn{to remove} \outofdate{The effects of using segmentation masks. a) We use the segmentation mask to extract the input training patches and to constrain the local loss on foreground object. The results contain well-propagated texture and no bleeding artifacts. b) If we only use segmentation mask for the input patch extraction but use global losses (applied to the entire image), we observe color and texture bleeding artifacts. c) If we turn off segmentation masks completely, the network converges much slower. Note that segmentation masks are never used at test time.}}
  \label{fig:dtd-segmentation-effect}
\end{figure}

==> figures/fig-RGBversusLAB.tex <==
\begin{figure}[htb]
  \centering
  \includegraphics[width=\linewidth]{images/RGB_LAB.pdf}
  \caption{\patsorn{to remove}\outofdate{Comparison between models trained on $\mathbf{RGB}$ versus $\mathbf{Lab}$. Enforcing feature, texture and adversarial losses on the $\mathbf{L}$ channel and adding a separate color loss on the $\mathbf{ab}$ channels significantly improve the color propagation.} }
  \label{fig:RGBversusLAB}
\end{figure}

%\patsorn{https://goo.gl/hzL0CR}

==> figures/fig-color-control.tex <==
\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{images/color_control.png}
  \caption{\patsorn{can we just remove this and put in supplementle or something} Results showing that the ab channel of our model can generalize well to user input}%Show results of controlling color using color patch by setting ab value of the texture patch to a certain value \patsorn{(optionally we will add scribbler stroke as another controlling option, we can also try stroke with the current model) https://goo.gl/P6ddf4}}%. 1.  result of general training using the color information in the groundtruth texture patch. 2. with the same sketch and texture patch, but different color channels for the texture patch. *3. same sketch and texture patch, no color channels for the texture patch, but use colored scribbles of colors different from ground truth.https://goo.gl/P6ddf4}
  \label{fig:color-control}
\end{figure}

==> figures/fig-dtd-results.tex <==
\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{images/placeholder.jpg}
  \caption{Applying textures from the DTD dataset held out from training. Show results on both clothes dataset and handbag dataset.}
  \label{fig:dtd-results}
\end{figure}

==> figures/fig-network-architecture.tex <==
\begin{figure}[htb]
  \centering
  \includegraphics[width=\linewidth]{images/placeholder.jpg}
  \caption{\patsorn{placeholder, to update. Network architecture. just a diagram or table showing layer details etc.} }
  \label{fig:network-architecture}
\end{figure}

==> figures/fig-patchsize-effect.tex <==
\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{images/placeholder.jpg}
  \caption{\patsorn{to update. replace with patch size/number/location experiment during test time} \outofdate{The effect of varying input patch sizes on training. Top row: At test time, the user can specify texture patches of different size. a) The network trained with fixed patch size of 30x30 cannot propagate the input texture. b) The network trained with varying patch sizes (20, 30, 40 or 50) better propagates the textures. }}
  \label{fig:patchsize-effect}
\end{figure}

%\patsorn{ https://goo.gl/jc6aWO}

==> figures/fig-results-clothing.tex <==
\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{images/placeholder.jpg}
  \caption{\patsorn{Show generalization to hand drawn sketch by training on multiple styles. Try showing how useful this application can be in real life ... }}
  \vspace{-2mm}
  \label{fig:results-clothing}
\end{figure}

==> texture_generalization.tex <==
\section{TextureGAN Generalization}
\label{sec:texture-generalization}
%\patsorn{emphasize better texture propagation}

One of the problem of training with ground truth image is that the network did not learn specifically to 'texturize' the object. It only learn to reconstruct the ground truth image by making use of all the hints we gave them during training. This create several problems: first, the real texture user want to apply is not always align with the information from sketch , secondly the ground truth image is not always rich enough in texture detail, often consist of image


%In our objective function, we decompose the target image into several components such as content, texture and color. During training, we compare these components with the ground truth image under the assumption that all those components comes from the same image. 
This works well for general texture that usually appear in the object naturally. However, when face with uncommon texture pattern, the network fails to generalize well \patsorn{provide an example. A side-by-side comparison of a result before DTD training and after DTD training}. In this section, we explore another option of using separate texture image to control texture of the output.

\subsection{Training data}
For training with separated texture images, we use texture dataset from Describable Textures Dataset [DTD] which consist of 120 texture categories each having around 47 texture images. We withheld 1 image per each categories and 32 texture categories for testing. We use the 110 images per category for training, 3688 in total. 

%\patsorn{check what exactly are we using}

\textbf{Localized Texture Loss Using Segmentation Mask. }
Naively using texture image for texture loss leads to a bleeding problem, because the network simply optimize for the same texture everywhere including the background. To avoid that, we utilize segmentation to locate where the object is and only apply texture to the object. This can be done as part of the objective function and doesn't require segmentation to be provided during testing. The objective function then becomes:

[objective function where texture loss only come from inside object boundary]

However, because the texture loss is based on feature extracted from pre-trained network (which is not a linear transformation), applying a mask to this feature is not straight forward because vgg network was trained on a full image, and the receptive field would get larger as the layer goes higher. [perceptual factor paper] create feature mask by downsampling the mask to the same size as the feature map, or identifying the node which the receptive field fall inside object boundary.
%they actually have to sort of erode over the feature mask so that they only left with the node that are looking only directly inside the boundary area.
This however is still not ideal due to overlapping receptive field, especially in the high level layer.

\textbf{Localize texture loss} we proposed using a localize texture loss where the loss only applied to small region in the image. Using information from the segmentation mask, we can ensure that the local loss patch will always be within object boundary (figure x). We randomize the location of the loss patch, and propagate  texture loss part of the object function only through that region of the output, while keeping the rest of the objective the same as before. 
%for reference feature size after passing local patch of 50 to vgg relu3 is 13x13
\cynthia{According to Patsorn, we use 1 fixed-size texture patch of size 100x100 for input resolution 256 or 60x60 for input resolution 128 to calculate the texture loss. The texture patch is required to overlap with the foreground object more than 70 percents. The original resolution of the DTD dataset is 512x512. We resize the textures to the input resolution of the network. When calculating the local texture loss, we crop random patches from the input texture and compare its the statistics with the output patch.}

\textbf{Background Loss}
With segmentation mask, we can also put more weight on the background part of the pixel loss, both in the L and ab channel. Doing so will penalize the network for bleeding the object into the background without increasing the influence of pixel loss which could contradict with the adversarial loss.



==> training.tex <==
\section{TextureGAN Overview}

Along the line of Scribbler~\cite{sangkloy2016scribbler}, we would like to give users direct controls over the image synthesis process using generative adversarial network (GAN). 
%
To control the generated output, the user gives the network several `hints' that contain incomplete information. The job of the network is to interpret the `hints' and hallucinate missing details in a meaningful way. 

Similar to Scribbler~\cite{sangkloy2016scribbler}, one type of `hints' we support is rough sketches that delineate object boundaries. Sketches effectively control the generation of semantic contents, the overall shapes and shadings, but do not contain enough information to guide the generation of texture details, materials and patterns. 

The goal of TextureGAN is to introduce a new `hint' to the network that allows users to directly control the types of textures generated in different semantic regions. On top of sketch, the user can `drag' rectangular texture patches of arbitrary sizes into different sketch regions as additional input to the network. For example, the user can specify a striped texture patch for the shirt and a dotted texture patch for the skirt. The input patches guide the network to propagate the texture information to the relevant regions respecting region boundaries.

TextureGAN also allows users to more precisely control the colors in the generated result. One limitation of Scribbler is that the user's input color constraint in the form of~$\mathbf{RGB}$~scribbles need to fight with the network's understanding about the semantics, e.g., bags are mostly black and shoes are seldom green.  
%
To address this problem, we train the network to generate images in $\mathbf{LAB}$ color space. We convert the groundtruth images to $\mathbf{LAB}$, enforce the content, texture and adversarial losses only on the $\mathbf{L}$ channel and enforce a separate color loss on the $\mathbf{ab}$ channels. 
%
We show that combining the controls in this way allows the network to generate realistic photos closely following the user's color and texture intents without introducing obvious visual artifacts.

%To allow user to use the input to control the output of the network, we essentially give the network several `hint' with incomplete information such as sketch (which only contain object boundary), and partial image patch (which only contain partial detail of the original image).
\input{figures/fig-diagram.tex}

Figure~\ref{fig:diagram} shows our training pipeline. 
%
We use the network architecture proposed in Scribbler~\cite{sangkloy2016scribbler}. 
%
We also use a 4-channel image as input to the network, but we change the channel specifications to support three different types of controls -- one channel for sketch, one channel for texture and two channels for color. Section~\ref{sec:training-data} describes the method we used to generate each input channel of the network.

We first train TextureGAN to recover the ground-truth photos given the synthetically generated input control channels. We train the generator to directly produce images in $\mathbf{LAB}$ space and then convert them to $\mathbf{RGB}$ space for the final results. Section~\ref{sec:losses} introduces the losses we use. We apply feature loss, adversarial loss and texture loss to the $\mathbf{L}$ channel and color loss to the $\mathbf{ab}$ channels.
%
To generalize TextureGAN to support broader range of textures, we fine-tune the network trained with ground-truth with a separate database, Describable Textures Dataset (DTD)~\cite{cimpoi14describing}. Section~\ref{sec:texture-generalization} describes how we modify the network training and losses to achieve the generalization goal.

%\cynthia{Mention the input and output of the network. talk about LAB versus RGB, use of different losses to improve texture generation. }
%The input to our network is a 4-channel image.  consist of 1 binary sketch, and 3 LAB channels of texture patch. Working on LAB color space allow us to separate color channels and optimize them separately in the objective function.
%\cynthia{mention the generator output is in LAB format somewhere.}

%\input{figures/fig-trainingdata.tex}

\section{Training Data Generation}
\label{sec:training-data}

We train TextureGAN on three object-centric datasets, handbags~\cite{isola2016image}, shoes~\cite{yu2014fine} and clothes~\cite{ATR,liang2015human}. They are similar in the way that the photo collections contain large variations of colors, materials and patterns. Precisely controlling the generation of textures is highly desirable for the scenarios of product design. For supervised training, we need to generate (input, output) image pairs. For the output of the network, we convert the ground-truth photos to $\mathbf{LAB}$ color space. For the input to the network, we process the ground-truth photos to extract 4-channel images. The four channels include one channel for the binary sketch, one channel for the texture patches and two channels for the color controls.

%\subsection{Generating training data}

\textbf{Sketch. }
%\subsection{Sketch} 
For \textbf{handbag and shoes}, we generate sketches using the deep edge detection method described in pix2pix~\cite{isola2016image}.
%
For \textbf{clothes}, we leverage the clothes parsing information provided in the dataset~\cite{ATR,liang2015human}. We apply Canny edge detection on the clothing segmentation mask to extract the segment boundaries as sketch. Different from the sketch generation method proposed by Scribbler~\cite{sangkloy2016scribbler}, we generate much simpler sketches that contain only the general outlines but no object details. We also process the ground-truth photos to white out the background.
%
%Figure~\ref{fig:trainingdata} shows some example sketches from the different categories.

\textbf{Texture Patches. }
%\subsection{Texture Patches}
%\label{sec:texture-patches}
%\cynthia{Talk about segmentation mask?}
To generate texture patches, we randomly crop small regions of the ground-truth image. In order to generate meaningful texture patches, we apply some heuristics to encourage putting crop regions inside the foreground object. We calculate the foreground object masks by applying the hole filling function of OpenCV~\cite{HoleFilling} on the sketches. We randomly choose the patch location and patch size and evaluate whether the patch overlaps the foreground object more than 70 percent of the time. If not, we randomly choose another location for the patch and reduce the patch size until the overlapping condition is satisfied. We convert each texture patch to the $\mathbf{LAB}$ color space and take the $\mathbf{L}$ channel only. We discretize the $\mathbf{L}$ channel values using integer numbers from 0 to 100.

%We treated the texture input to the network as discrete integer number, ranging from 0-100 on lightness channel, and -128 to 128 on the ab channels. Because our partial texture patch wont be taking the entire area of the input, we specify the mask by using non-valid pixel value (i.e. negative value outside of the range). We randomize the size and location of the patch, but make it more likely to be generated inside object boundary rather than outside.

We generate one texture patch for \textbf{handbag and shoes}, and two patches for \textbf{clothes}. For clothes, we extract two patches from two different semantic regions -- top, skirt, pant, dress, bag or scarf. For the regions outside the mask, we use an invalid pixel value (i.e. negative value outside of the range).

%\cynthia{describe heuristics of extracting patch within object boundary. not important for groundtruth, but important for DTD training.}

\textbf{Color Patches or Scribbles. }
%\subsection{Color Patches or Scribbles}
%\patsorn{@Cynthia, you are right, i don't think we need this part. let keeps the color controlling part in the result, but use patch ab channel to control color }
To give users control on the generated color, we support two types of color input, color patches or color scribbles. For color patches, we determine its location and size in the same way as texture patches. We take the $\mathbf{ab}$ channels of the ground-truth patch as values for the color patch. We discretize the $\mathbf{ab}$ values using an integer ranging from -128 to 128. For regions outside the color patch, we set the pixel values to be -200 (invalid value outside the valid $\mathbf{ab}$ range.
%
At run-time, specifying color patches might be hard for small and narrow objects. Therefore we also allow scribble strokes as color constraints. To extract color scribbles for training, we follow the method introduced by Scribbler~\cite{sangkloy2016scribbler}. Unless specified otherwise, all results shown in the paper are produced by models trained with color patches. 

Figure~\ref{fig:ablation-study}, \ref{fig:patchsize-effect}, \ref{fig:RGBversusLAB}~and~\ref{fig:color-control} show some example inputs to the network. Note that the color patches and the texture patches are placed at the same locations.

%With the current training pipeline, we can actually control color of the texture via AB channel of the input. Using color `patch' is inconvenient however, and also limiting since it only allow control of the texture color. To control color of the output image, we follow the approach proposed in [Scribbler]--training with color stroke to simulate user interaction for controlling color. However, instead of using RGB as proposed in [Scribbler] which is proned to color conflicting when combine with adversarial loss, we operate instead in LAB color space. We synthetically generate the color stroke based on color from the ground truth image, and use as input to the AB channel of the network. 

\section{TextureGAN Training}
\label{sec:losses}
We aim to replicate the texture information contained in small patches to fill in an entire object. 
%
We find that the losses used in Scribbler are not sufficient for this purpose. 
%
Scribbler's feature loss and adversarial loss encourage the generation of realistic object structures and colors, but cannot reproduce the fine-grained texture details. 
%
Their pixel loss encourages the generated image to follow the input color constraints, but fails when the input color is rare for the particular object category. 
%
Therefore, we need to redefine the losses to improve the replication of texture details and encourage precise propagation of colors. 
%
Note that all input channels to the network are derived from ground-truth photos. When computing the losses, we compare the generated images with the ground-truth photos.
%
Our objective function consists of multiple terms, each of which encourages the network to focus on different aspects. 

%We expect the network to correctly interpret each input constraint, therefore it is important to define the losses that specifically encourages the generation of contents, replication of textures and propagation of colors. 

%We expect the network to learn to associate each part of the input constrain to the correct output. Therefore it's very important to define the `right' output via the objective function that we want the network to optimize for. 
%Although there's only one right image (for now. we explore using separate texture image in section x), how we represent such image can affect how the network learn, i.e. if we only using pixel loss, getting the right background is equally important as getting the right object shape, which is not what we want 


%\cynthia{Talk about why use LAB space and why training content, texture and adversarial loss all in LAB space.}

\textbf{Feature Loss. }
It has been shown previously that the features extracted from middle layers of a pre-trained neural network, VGG-19~\cite{simonyan2014very}, represent high-level semantic information of an image~\cite{guccluturk2016sketchinv, sangkloy2016scribbler}. Given a rough outline sketch, we would like the generated image to loosely follow the object structures specified by the sketch. Therefore, we decide to use a deeper layer of VGG-19 for feature loss (relu 4\_2). To focus the feature loss on generating structures, we convert both the ground-truth image and the generated image from $\mathbf{RGB}$ color space to $\mathbf{LAB}$ and generate grayscale images by repeating the $\mathbf{L}$ channel values. We then feed the grayscale image to VGG-19 to extract features. The feature loss $\mathcal{L}_{f}$ is defined as the L2 difference in the feature space. During back propagation, the gradients passing through the L channel of the output image are averaged from the three channels of the VGG-19 output. 
%\cynthia{I am not quite sure what the previous sentence means}
%When user draw a sketch, we expect the network to generate an image with corresponding content. It has been shown that the output activation extract from a classification network can capture high level semantic information of the image. Therefore, we define a feature loss as 
%\cynthia{question: the output of the network is a LAB image?}

%[feature loss]

%where we use vgg-19 network, trained on ImageNet to encode raw rgb image into meaningful feature representation (extracted from layer relu 4\_2). We again disregard color by optimizing content loss only on greyscale image. Since vgg-19 was trained on RGB, we convert greyscale image from L channel output into RGB  before extracting feature. We average gradient from the 3 channels and only backprop through the L channel output. This also help separate color from the content image, which will be useful when we want color to come from a separate image (section x). 

%By optimizing for feature loss, we emphasize on the importance of matching the right 'content'. 

%To encourage the network to generate image that correspond to the sketch, we define content loss as the loss that penalize when the results deviate from the gt image (that prompt the sketch and texture patch) in various aspect. 

\textbf{Adversarial Loss. }
%\subsubsection{Adversarial Loss}
%\label{sec:adversarial-loss}
Generative adversarial network (GAN) has been shown to be able to generate realistic images from random noises~\cite{goodfellow2014generative}. 
%
In GAN, a generator network and a discriminator network are trained simultaneously in a minimax game. The discriminator tries to tell apart generated images from real photos while the generator tries to generate realistic images tricking the discriminator into thinking they are real. By alternating the optimization of the generator and the discriminator until convergence, the generator can generate images indistinguishable from real photos. 
%Recently GAN has shown to be very promising in constraining the generative results to be indistinguishable from real image (as seen from the perspective of the discriminator). 
%
%In general, the adversarial training is very unstable, due to the difficulty of optimizing two opposing networks. Because of the instability, GAN is usually used as a standalone objective function, where the goal is to simply generate realistic image from random noise. 
%

In recent work, the concept of adversarial training has also been adopted  in the context of image to image translation. In particular, one can attach a trainable discriminator network at the end of the image translation network and use it to constrain the generated result to lie on the training image manifold. Previous work proposed to minimize the adversarial loss (loss from the discriminator network) together with other standard losses (pixel, feature losses, etc). The exact choice of losses depends on the different applications~\cite{sangkloy2016scribbler, isola2016image, guccluturk2016sketchinv}. 
%
Our work follows the same line. We use adversarial loss on top of feature, texture and color losses. The adversarial loss pushes the network towards synthesizing sharp and realistic images, but at the same time constrains the generated images to choose among typical colors in the training images. The network's understanding about color sometimes conflicts with user's color constraints, e.g. an user provides a rainbow color constraint for a handbag, but the adversarial network thinks it looks fake so refuses to generate such output. 
%\cynthia{Give an example showing that adversarial network does not generate the colors user wants.}
%In the context of image to image translation, GAN has been integrated into the training as adding an adversarial loss on top of other standard losses that encourage the resulting previous work integrated the GAN concept into the training by adding adversarial loss on top of other standard losses (pixel, feature losses, etc) to improve the sharpness and realism of the resulting images~\cite{sangkloy2016scribbler, isola2016image, guccluturk2016sketchinv}. 
%(I call it 'discriminator loss', but it's actually a generator loss that compute from the gradient of the discriminator, so we might want to define that or something) 
%The purpose of the adversarial loss is to push the network toward synthesizing sharp and realistic images. 
%, which is useful especially for our problem where the sketch could have has many valid image corresponding to it. 
%The discriminator loss would favor the one that look most realistic. This however, create a problem where what the discriminator consider realistic might be conflicting with our user constrain, especially in color domain i.e. user want a rainbow handbag, but the network think it looks fake so it refuse to output that. [example]
%Although the discriminator is useful for making sure the object color is realistic, there's not much else the discriminator could contribute in the color domain. 
Therefore, we propose applying the adversarial loss $\mathcal{L}_{adv}$ only on greyscale image (repeating the $\mathbf{L}$ channel in $\mathbf{LAB}$ space). The discriminator is trained to disregard the color but focus on generating sharp and realistic details. The gradients of the loss only flow through the $\mathbf{L}$ channel of the generator output. This effectively reduces the search space and makes GAN training easier and more stable. 
%
We perform the adversarial training using the techniques proposed in DCGAN~\cite{radford2015unsupervised} with the modification proposed in LSGAN~\cite{mao2016least}. LSGAN proposed replacing the cross entropy loss in the original GAN with linear least square loss for higher quality results and stable training.

%, or where the discriminator might be recognizing right/wrong image in addition to just real/fake (ex. the right image could be the image that correspond to the input caption [cite]). But the advantage of GAN is their ability to approximate any distribution, even that of natural image (which is tricky to do so directly, since we don't know how to model natural image). And that's exactly how we use GAN in our problem-- to make the output looks more realistic. 

\textbf{Texture Loss. }
%\subsubsection{Texture Loss}
%\label{sec:texture-loss}
In addition to generating the right content following the input sketch, we would also like to propagate the texture details given in the input texture patch. The previous feature and adversarial losses are unable to capture fine-scale details, since they focus on getting the overall structure correct. 
%
Similar to deep learning based texture synthesis and style transfer work~\cite{gatys2015texture, gatys2015neural}, we use style loss to specifically encourage the reproduction of texture details. We adopt the idea of matching the Gram matrices (feature correlations) of the features extracted from certain layers of the pretrained classification network (VGG-19). The Gram matrix $\mathcal{G}^{l}_{ij} \in 
\mathcal{R}^{{N}_{l}x{N}_{l}}$ is defined as:
%
\begin{equation}\label{eq:gram-matrix}
\mathcal{G}^{l}_{ij} = \sum_{k}\mathcal{F}^{l}_{ik}\mathcal{F}^{l}_{jk}
\end{equation}
%
where, $N_l$ is the number of feature maps at network layer $l$, $\mathcal{F}^{l}_{ik}$ is the activation of the $i$th filter at position $k$ in layer $l$. 
%It has been shown that a set of Gram matrices $\{\mathcal{G}^{l_1}, \mathcal{G}^{l_2}, ...\}$ from some layers $l_1$, $l_2$, ..., in the network is a good texture descriptor~\cite{gatys2015texture, gatys2015neural}. 
We use two layers of the VGG-19 network (relu3\_2, relu4\_2) to define our style loss, $\mathcal{L}_s$. 

On top of that, we find that adding certain amount of L2 pixel loss $\mathcal{L}_p$ stabilizes the training and leads to the generation of more texture details faithful to the user's input texture patch. So we define the overall texture loss as: $\mathcal{L}_{t} = \mathbf{w}_p\mathcal{L}_p + \mathcal{L}_s$, where $\mathbf{w}_p$ is fixed to be 10. Similar to the feature and adversarial losses, the texture loss is enforced only on the grayscale images. 

%\cynthia{Add discussion of histogram loss if the training if it is done in time.}
%\cynthia{Mention the weight of the pixel loss versus style loss. Pixel weight is 10 times the style weight.}


%In addition to getting the right content, we also want to get the right texture details corresponding to the input texture patch. This information is unlikely to get capture by the previous feature loss of especially that of higher level layer. The most straight forward loss for such detail would be simply using pixel loss, which would encourage the network to recreate exactly the original image. However, we found that it is more helpful to have another term of the loss that emphasize more on matching texture statistic.
%Recently, there are several attempt at texture synthesis via deep learning based approach [cite]. 
%The main idea is that it is possible to capture style/texture statistic by using gram matrix (outer product) of the feature extracted from classification network. 
\cynthia{Tone down texture loss since it does not seem to help too much.}
\patsorn{Texture loss seems to help a lot with dtd training, so we might want to shift the focus of texture loss there.}

\textbf{Color Loss. }
%\subsubsection{Color loss}
%\label{sec:color-loss}
As described above, we intentionally apply feature, adversarial and texture losses on only the $\mathbf{L}$ channel of the output to focus them on generating sketch-conforming structures, realistic shadings and sharp high-frequency texture details. To enforce the user's color constraints, we add a separate color loss $\mathcal{L}_{c}$ that penalizes the L2 difference between the $\mathbf{ab}$ channels of the generated result and that of the ground-truth. 
%We also ensure color matching by adding separated pixel loss for ab channels of the output. Where,
%[AB\_loss = l2 on ab]
We find that the color loss is effective in propagating colors regardless of the types of color inputs, patches or scribbles. \patsorn{depends on if we have scribble stroke option, }

%We also explored using different types of color control via scribbler stroke.

%With the current training pipeline, we can actually control color of the texture via AB channel of the input. Using color `patch' is inconvenient however, and also limiting since it only allow control of the texture color. To control color of the output image, we follow the approach proposed in [Scribbler]--training with color stroke to simulate user interaction for controlling color. However, instead of using RGB as proposed in [Scribbler] which is proned to color conflicting when combine with adversarial loss, we operate instead in LAB color space. We synthetically generate the color stroke based on color from the ground truth image, and use as input to the AB channel of the network. 

Our combined objective function is defined as:
%
\begin{equation}\label{eq:objective-function}
\mathcal{L} = \mathcal{L}_{f} + \mathbf{w}_{adv}\mathcal{L}_{adv} + \mathbf{w}_{t}\mathcal{L}_{t} + \mathbf{w}_{c}\mathcal{L}_{c}
\end{equation}
%
The exact training details can be found in section~\ref{sec:training-details}.



%Initially, the gradient from the discriminator would not be informative yet due to the output being quite noisy in early stage. We find it helpful to turn off the discriminator loss initially, and optimize for the rest of the objective function until converging. Adding discriminator afterward allows the network to focus mostly on optimizing the discriminator loss, while keeping the rest of the objective stable. Using this trick we can train the discriminator loss along side other objective function without adding much instability to the training.

%We provide more detail of the training parameters for each of the category in the supplementary material.
%\cynthia{Are we really going to have a supplementary material? If not, we should add important details to the paper itself.} \patsorn{it's not a single number we can report, each models actually use different parameters, we did record all those, like when did we start using discriminator, or change weight and such so hopefully we'll have all the detail for reproducibility but i'm not sure it's gonna fit here >,<}

%\cynthia{mention the relative weights of different losses}
%\patsorn{add any trick/tip/insight/interesting behavior we have for the training, Amit and Wenqi might have something more to add}

%\patsorn{one interesting thing we can note is that when increasing the resolution of the input, the network end up choosing either L channel or AB channel to optimize and ignore the other. maybe link to possible future work that we can tweak the network architecture (dilate conv) or maybe use a two-steam or two-branch network that has separate subnetwork dealing with separate loss. }

%% color control
%We start with the network that was trained earlier, and fine tune to these augmented training data. The final network is able to generate output that match all three input constrains--sketch, texture, and color. [figure for examples]

